Training Dynamics of Multi-Head Softmax Attention for In-Context Learning: Emergence, Convergence, and Optimality

We study the dynamics of gradient flow for training a multi-head softmax attention model for in-context learning of multi-task linear regression. We establish the global convergence of gradient flow under suitable choices of initialization. In addition, we prove that an interesting "task allocation" phenomenon emerges during the gradient flow dynamics, where each attention head focuses on solving a single task of the multi-task model. Specifically, we prove that the gradient flow dynamics can be split into three phases -- a warm-up phase where the loss decreases rather slowly and the attention heads gradually build up their inclination towards individual tasks, an emergence phase where each head selects a single task and the loss rapidly decreases, and a convergence phase where the attention parameters converge to a limit. Furthermore, we prove the optimality of gradient flow in the sense that the limiting model learned by gradient flow is on par with the best possible multi-head softmax attention model up to a constant factor. Our analysis also delineates a strict separation in terms of the prediction accuracy of ICL between single-head and multi-head attention models. The key technique for our convergence analysis is to map the gradient flow dynamics in the parameter space to a set of ordinary differential equations in the spectral domain, where the relative magnitudes of the semi-singular values of the attention weights determines task allocation. To our best knowledge, our work provides the first convergence result for the multi-head softmax attention model.

==> sections/dynamics.tex <==
\section{Training dynamics under Rotation Invariance Condition}


\subsection{Gradient flow}
% Let us define $\frac{\partial \ell}{\partial \hat y_q^h} = \partial \ell / \partial \hat y_q^h \in\RR^{1\times d_y}$ as the gradient of the loss with respect to the output of each head.
During the training,  the backward information is given by 
\begin{align*}
    % \frac{\partial \ell}{\partial \hat y_q^h} &= \frac{\partial \ell}{\partial \hat y_q^h}, 
    % \tag*{\# shape: $[1, d_y]$ }\\
    \frac{\partial \ell}{\partial p^h} &= \frac{\partial \ell}{\partial \hat y_q^h} O^h V^h Z,
    \tag*{\# shape: $[1, L]$ }\\
    \frac{\partial p^h}{\partial s^h} &= \diag(p^h) - p^h (p^h)^\top \eqdef \KK^h, 
    \tag*{\# shape: $[L, L]$ }
\end{align*}
where the shape of $\partial\ell / \partial \hat y_q^h$ is $[1, d_y]$.
Therefore, 
\begin{align*}
    \dot O^h &= - \underbrace{\EE\left[ \left(\frac{\partial \ell}{\partial \hat y_q^h}\right)^\top (p^h)^\top Z^\top\right]}_{\ds B^h} (V^h)^\top = - B^h (V^h)^\top,
    \tag*{\# shape: $[d_y, d]$ }\\
    \dot V^h &= -(O^h)^\top  \EE\left[ \left(\frac{\partial \ell}{\partial \hat y_q^h}\right)^\top (p^h)^\top Z^\top \right] = - (O^h)^\top B^h,
    \tag*{\# shape: $[d, D]$ }\\
    \dot K^h &= - \frac 1 {\sqrt{d}} Q^h \EE \left[  z_q \frac{\partial \ell}{\partial \hat y_q^h} O^h V^h Z \KK^h Z^\top \right] = - \frac 1 {\sqrt{d}} Q^h (A^h)^\top, 
    \tag*{\# shape: $[d, D]$ }\\
    \dot Q^h &= - \frac 1 {\sqrt{d}} K^h \underbrace{\EE\left[Z \KK^h Z^\top (O^h V^h)^\top \left(\frac{\partial \ell}{\partial \hat y_q^h}\right)^\top z_q^\top\right]}_{\ds A^h} = - \frac 1 {\sqrt{d}} K^h A^h, 
    \tag*{\# shape: $[d, D]$ }
\end{align*}
where we define $A^h$ and $B^h$ as the expectation terms in the above equations.
We consider $\ell(\hat y_q, y_q) = \|\hat y_q - y_q\|^2/2$. Therefore, $\frac{\partial \ell}{\partial \hat y_q^h} = (\hat y - y)^\top = (\sum_{h'=1}^H O^{h'} V^{h'} Z p^{h'} - y_q)^\top$. One might notice that the output of different attention heads are correlated. However, we are able to show that the correlation does not exists under proper initialization. For simplicity, we use the notations $W^h = (K^h)^\top Q^h / \sqrt{d}$ and $U^h = O^h V^h$ in the sequel.

\subsection{Properties of the Dynamics}
In this subsection, we characterize some basic properties of the dynamics. 
The first property we aim to show is that the $X$ parts and the $Y$ parts are decoupled in the dynamics, which can help simplify the analysis.

\begin{definition}[Uncoupling of $X$ and $Y$] \label{def:uncoupling X Y property}
    We say that a set of parameters $\{O^h, V^h, K^h, Q^h\}_{h=1}^H$ uncouples $X$ and $Y$ if the following four conditions hold
    \begin{itemize}
    % \begin{steps}
        \item[(i)] $\col(V_{Y}^h) \perp \col(V_{X}^{h})$ for all $h\in[H]$.
        \item[(ii)] $\row(O^h) \subseteq \col(V_{Y}^h)$ for all $h\in[H]$.
        \item[(iii)] $\col(K_{ Y}^h) \perp \col(K_{X}^h)$ for all $h\in[H]$.
        \item[(iv)] $\col(Q_{ X}^h) \subseteq \col(K_{X}^h)$ for all $h\in[H]$.  
    \end{itemize}
    Here, we use the notation $V_{X}^h$ to denote the $X$ part of $V^h$, i.e., $V_{X}^h = V^h[:, 0{:}d_x]$, and $V_{ Y}^h$ to denote the $Y$ part of $V^h$, i.e., $V_{ Y}^h = V^h[:, d_x{:}]$. The notations $K_{ X}^h$, $K_{ Y}^h$, $Q_{ X}^h$ and $Q_{ Y}^h$ are defined similarly.
\end{definition}
Moreover, the following proposition shows that this uncoupled property are invariant under the gradient flow.
\begin{proposition}\label{prop: uncoupling dynamics}
    If the initialization satisfies the uncoupling property for $X$ and $Y$ defined in \Cref{def:uncoupling X Y property}, then the following properties hold during the gradient flow:
    \begin{itemize}
        \item[(i)] The uncoupling property in \Cref{def:uncoupling X Y property} is preserved.
        \item[(ii)] $p^h\indep Y$.
        \item[(iii)] $V_{ X}$, $K_{ Y}$ and $Q_{ Y}$ will be fixed at initialization.  
    \end{itemize}
\end{proposition}
\begin{proof}
    Let $U^h = O^h V^h$ and $W^h = (K^h)^\top Q^h$. We show that under the uncoupling property \Cref{def:uncoupling X Y property}, we have $U_X^h = 0$ and $W_{Y, X}^h = 0$, where $U_X^h = U_X^h[:, 0{:}d_x]$ and $W_{Y, X}^h = W^h[d_x{:}, 0{:}d_x]$. This is just a matter of matrix calculation. 
    \begin{align*}
        U_X^h = O^h V_{X}^h = 0, \quad W_{Y, X}^h = (K_{ Y}^h)^\top Q_{ X}^h = 0.
    \end{align*}
    The first equality holds since $ \row(O^h) \subseteq \col(V_{Y}^h)$ and $\col(V_{Y}^h) \perp \col(V_{X}^h)$, and the second equality holds since $\col(Q_{ X}^h) \subseteq \col(K_{X}^h)$ and $\col(K_{ Y}^h) \perp \col(K_{X}^h)$.
    We next show that the four conditions in \Cref{def:uncoupling X Y property} are preserved under the gradient flow.

\paragraph{Calculation of $B^h$ and Independence of $p^h$ and $Y$.}
We start with calculating $B^h$. We have by definition that
\begin{align*}
    B^h &= \EE \left[  \left(\sum_{h'=1}^H O^{h'} V^{h'} Z p^{h'} - y_q\right) (Z p^h)^\top \right] \\
    &= \EE \left[ \sum_{h'=1}^H O^{h'}V^{h'} Z p^{h'} (Z p^h)^\top \right] - \EE \left[ y_q (Z p^h)^\top \right] \\
    &= \sum_{h'=1}^H O^{h'} V^{h'} \EE\left[
         \left(\begin{pmatrix}I_{d_x} \\\beta^\top\end{pmatrix} X + \begin{pmatrix} 0\\ \varepsilon\end{pmatrix}\right) p^{h'} (p^h)^\top \left(X^\top \begin{pmatrix} I_{d_x} , \beta \end{pmatrix}+ \begin{pmatrix} 0, \varepsilon^\top \end{pmatrix}\right)
    \right] \\
    &\qquad
    - \EE\left[
        \beta^\top x_q (p^h)^\top \left(X^\top \begin{pmatrix} I_{d_x} , \beta \end{pmatrix}+ \begin{pmatrix} 0, \varepsilon^\top \end{pmatrix}\right) 
    \right].
    % \bluetag{$p^h \indep \beta, \varepsilon$}
\end{align*}
A simple rearrangement gives
\begin{align}
    B^h &= \sum_{h'=1}^H O^{h'} V^{h'} \EE\begin{pmatrix}
        X p^{h'}(p^h)^\top X^\top & X p^{h'}(p^h)^\top X^\top \beta \notag\\
        \beta^\top X p^{h'}(p^h)^\top X^\top & \beta^\top X p^{h'}(p^h)^\top X^\top \beta + \varepsilon p^{h'}(p^h)^\top \varepsilon^\top
    \end{pmatrix} \notag\\
    &\qquad
    - \EE\left[
        \beta^\top x_q (p^h)^\top X^\top \begin{pmatrix} I_{d_x} , \beta \end{pmatrix}
    \right] 
    \bluetag{$\varepsilon\indep (p^h, \beta, x_q)$} \notag\\
    & = \sum_{h'=1}^H \EE\begin{pmatrix}
        O^{h'} V_{ X}^{h'}X p^{h'}(p^h)^\top X^\top, & 
        O^{h'} V_{ Y}^{h'} \left(\beta^\top X p^{h'}(p^h)^\top X^\top \beta + \varepsilon p^{h'}(p^h)^\top \varepsilon^\top \right)
    \end{pmatrix} \bluetag{$\EE[\beta]=0, \beta\indep (X, p^h)$}\\
    &\qquad
    -
         \begin{pmatrix} 0 , & \EE\left[\beta^\top x_q (p^h)^\top X^\top\beta\right] \end{pmatrix} , 
    \label{eq: B^h-1}
\end{align}
where in the first equality, we use the fact that $\varepsilon$ is an independent noise and in the second equality, we use the fact that $\EE[\beta]=0$ to get rid of the cross terms. Note that what is inherited in this reduction is the independence between $p^h$ and $(\beta, \varepsilon)$. 
This is in fact guaranteed by the uncoupling property $W_{Y, X}^h =0$. To see this point, we note that the attention score $s_l^h$ is given by 
$$s_l^h = z_l^\top W^h z_q = z_l^\top W_{:, X}^h x_q = x_l^\top W_{X, X}^h x_q + y_l^\top W_{Y,X}^h x_q = x_l^\top W_{X, X}^h x_q.$$
where the second equality holds since $z_q$ has zero in the last $d_y$ entries, and the last equality holds by the conclusion of the uncoupling property that $W_{Y, X}^h = 0$. 

\paragraph{Preservation of condition (i).}
We define $B_X^h = B^h[0{:}d_x, :]$. We have from \eqref{eq: B^h-1} that
\begin{align*}
        B_X^h = \sum_{h'=1}^H U_X^{h'} \EE\left[X p^{h'} (p^h)^\top X^\top\right] = 0, 
\end{align*}
which holds since we also have $U_X^{h} = 0$ for all $h\in[H]$. Recall from the dynamics that 
\begin{align}
    \dot V_{ X}^h = - (O^h)^\top B_X^h=0, \quad \dot V_{ Y}^h = - (O^h)^\top B_Y^h. \label{eq: dynamics of V^h-1}
\end{align}
Therefore, we have that $V_{ X}^h $ remains unchanged under the gradient flow. It is thus sufficient to show that during the gradient flow, $V_{ Y}^{h}$ has columns orthogonal to the columns of $V_{ X}^{h}$ at initialization. 

which implies that $\col(\dot V_{ Y}^h)\subset \row(O^h)\subset \col(V_{ Y}^h)$, meaning that the columns of $V_{ Y}^h$ are updated within the subspace spanned by the columns of $V_{ Y}^h$ at initialization. 
Since we already have $\col(V_{ Y}^h) \perp \col(V_{ X}^h)$ at initialization, such a property will be preserved under the gradient flow.

\paragraph{Preservation of condition (ii).}
We note that $\dot O^h = - B^h (V^h)^\top = - B_Y^h V_{ Y}^h$. As we have shown in the previous paragraph, $\col(V_{ Y}^h)$ remains unchanged under the gradient flow \footnote{Here, we say that the column space is \say{unchanged} even though the actual column space could be just a subspace of the original one at initialization, as long as $V_{ Y}^h$ does not go beyond the column space at initialization.}. Thus, $\row(O^h)$ remains a subset of $\col(V_{ Y}^h)$ under the gradient flow.


We show the preservation of the last two conditions by calculating $A^h$ in the following.
\paragraph{Calculation of $A^h$.}
Now, we deal with $A^h$. In the following, we let $U^h = O^{h} V^{h}$, $U_X^h = O^{h} V_{ X}^{h}$ and $U_Y^h = O^{h} V_{ Y}^{h}$. By definition, we have
\begin{align*}
    A^h &= \EE\left[Z \KK^h Z^\top (V^h)^\top \left(\sum_{h'=1}^H U^{h'} Z p^{h'} - y_q\right) z_q^\top\right] \\
    % plug in Z = (I;\beta^\top) X + (0;\varepsilon)
    &=\EE\left[
        \left(\begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X + 
        \begin{pmatrix}
            0 \\ \varepsilon
        \end{pmatrix}\right)
        \KK^h 
        \left(\begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X + 
        \begin{pmatrix}
            0 \\ \varepsilon
        \end{pmatrix}\right)^\top (U^h)^\top \left(\sum_{h'=1}^H U^{h'} \left(\begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X + 
        \begin{pmatrix}
            0 \\ \varepsilon
        \end{pmatrix}\right) p^{h'} - y_q\right) z_q^\top
    \right].
\end{align*}
We denote by $A^{h, h'}$ each term in the summation given by
\begin{align*}
    A^{h, h'} = \EE
    \left[
        Z \KK^h Z^\top (U^h)^\top U^{h'} Z p^{h'} z_q^\top
    \right], \quad A^{h, 0} = \EE\left[
        Z \KK^h Z^\top (U^h)^\top (-y_q) z_q^\top \right].
\end{align*}
For $A^{h, 0}$, it holds from $p^h\indep (\beta, \varepsilon)$ and $\beta\indep \varepsilon$ (which we have shown in the calculation of $B^h$) that 
\begin{align*}
    A^{h, 0} &= - \EE\left[
        \left(\begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix} X + \begin{pmatrix}
            0 \\ \varepsilon
        \end{pmatrix}\right)
        \KK^h \left(X^\top 
        \begin{pmatrix}
            I_d, & \beta
        \end{pmatrix} + \begin{pmatrix}
            0, & \varepsilon^\top
        \end{pmatrix}
        \right)
         (U^h)^\top \beta^\top x_q z_q^\top
    \right] \\
    & = -\begin{pmatrix}
        \EE\left[
            X \KK^h X^\top \beta (U_Y^h)^\top \beta^\top x_q z_q^\top
        \right] \\
        \EE\left[
            \beta^\top X \KK^h X^\top (U_X^h)^\top \beta^\top x_q z_q^\top 
        \right]
    \end{pmatrix}.
\end{align*}
For $A^{h, h'}$, it holds that
\begin{align*}
    A^{h, h'} &= \EE\left[
        \left(\begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X + 
        \begin{pmatrix}
            0 \\ \varepsilon
        \end{pmatrix}\right)
        \KK^h 
        \left(\begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X + 
        \begin{pmatrix}
            0 \\ \varepsilon
        \end{pmatrix}\right)^\top (U^h)^\top U^{h'} \left(\begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X + 
        \begin{pmatrix}
            0 \\ \varepsilon
        \end{pmatrix}\right) p^{h'} z_q^\top
    \right] \\
    % We use the fact that \varepsilon is independent noise and only keep the terms with degree 0 or 2 of \varepsilon
    &= \EE\left[
        \begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X 
        \KK^h X^\top 
        \begin{pmatrix}
            I_d, & \beta
        \end{pmatrix} 
         (U^h)^\top U^{h'} 
         \begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X p^{h'} z_q^\top
    \right] \\
    & \autoquad{2} + \EE\left[
        \begin{pmatrix} 
            0 & 0 \\
            0 & \varepsilon \KK^h \varepsilon^\top
        \end{pmatrix}
        (U^h)^\top U^{h'} \begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X
        p^{h'} z_q^\top
    \right]\\
    & \autoquad{2} + \EE\left[
        \begin{pmatrix} 
            0 \\
            \varepsilon \KK^h X^\top \begin{pmatrix}
            I_d, & \beta
            \end{pmatrix} (U^h)^\top U^{h'} \begin{pmatrix}
            0 \\ \varepsilon
        \end{pmatrix}
        p^{h'} z_q^\top
        \end{pmatrix}
    \right]\\
    & \autoquad{2} + \EE\left[
        \begin{pmatrix} 
            I_d \\ \beta^\top
        \end{pmatrix} X
        \KK^h \begin{pmatrix}
            0, & \varepsilon^\top
        \end{pmatrix} (U^h)^\top U^{h'} \begin{pmatrix} 
            0 \\
            \varepsilon
        \end{pmatrix}
        p^{h'} z_q^\top
    \right]
    \bluetag{$\varepsilon$ is independent noise}
    \\
    % We cancel out \beta except for the first term
    &= \underbrace{\EE\left[
        \begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X 
        \KK^h X^\top 
        \begin{pmatrix}
            I_d, & \beta
        \end{pmatrix} 
         (U^h)^\top U^{h'} 
         \begin{pmatrix}
            I_d \\ \beta^\top
        \end{pmatrix}
        X p^{h'} z_q^\top
    \right]}_{\dstext{(a)}} \\
    & \autoquad{2} + \EE\left[
    \begin{pmatrix} 
        X \KK^h  \varepsilon^\top
        (U_Y^h)^\top U_Y^{h'}\varepsilon
        p^{h'} z_q^\top 
        \\
        \varepsilon \KK^h \varepsilon^\top (U_Y^h)^\top U_X^{h'} X p^{h'} z_q^\top + \varepsilon \KK^h X^\top (U_X^h)^\top U_Y^{h'} \varepsilon
        p^{h'} z_q^\top
    \end{pmatrix}
    \right].
    \bluetag{$\beta$ is independent of $p$}
\end{align*}
Here, the first term is the signal term and the second term is the noise term. We can further decompose the signal term into two parts: the first part is the signal term without $\beta$ and the second part is the signal term with $\beta$. We have
\begin{align*}
    \dstext{(a)} = 
    \EE\left[
        \begin{pmatrix}
        X \KK^h X^\top (U_X^h)^\top U_X^{h'} X p^{h'} z_q^\top
        + X \KK^h X^\top \beta  (U_Y^h)^\top U_Y^{h'} \beta^\top X p^{h'} z_q^\top
            \\
        \beta^\top X \KK^h X^\top \beta (U_Y^h)^\top U_X^{h'} X p^{h'} z_q^\top + \beta^\top X \KK^h X^\top (U_X^h)^\top U_Y^{h'} \beta^\top X
        p^{h'} z_q^\top
        \end{pmatrix}
    \right]. 
\end{align*}
To this end, our main focus is the part of $A^h$ without $U_X^h$ or $U_X^{h'}$, as we have already shown that $U_X^h=0$. Define $A_X^h=A^h[0{:}d_x, :]$ and $A_Y^h=A^h[d_x{:}, :]$. We have
\begin{align}
    A_X^h &= \EE\left[ X \KK^h X^\top \beta  (U_Y^h)^\top \left( \sum_{h'} U_Y^{h'} \beta^\top X p^{h'} - \beta^\top x_q \right) z_q^\top \right] + \sum_{h'}\EE\left[X \KK^h  \varepsilon^\top
    (U_Y^h)^\top U_Y^{h'}\varepsilon
    p^{h'} z_q^\top\right]. \label{eq: A^h-1}
\end{align}
We also have $A_Y^h = 0$ following from the fact that $U_X^h =0$. 

\paragraph{Preservation of condition (iii).}
The idea here is similar to the preservation of condition (i). We show that $K_{ Y}^h$ remains unchanged and that $K_{ X}^h$ only updates within the subspace spanned by the columns of $K_{ X}^h$ at initialization.
Note that by the dynamics, 
\begin{align}
    \dot K_{ Y}^h = - \frac 1 {\sqrt{d}} Q^h (A_Y^h)^\top = 0, \quad \dot K_{ X}^h = - \frac 1 {\sqrt{d}} Q^h (A_X^h)^\top = - \frac 1 {\sqrt{d}} Q_{ X}^h (A_{X, X}^h)^\top, \label{eq: dynamics of K^h-1}
\end{align}
where we define $A_{X, X}^h = A^h[0{:}d_x, 0{:}d_x]$. 
Here, the first equality holds since $A_Y^h = 0$ and the second equality holds since $A_X^h$ has the last $d_y$ columns being zero guaranteed by the zeros in the last $d_y$ entries of $z_q$.
Therefore, $\col(K_{ Y}^h)$ remains unchanged under the gradient flow.
In addition, $\col(\dot K_{ X}^h) \subseteq \col(Q_{ X}^h) \subseteq  \col(K_{ X}^h)$. Therefore, the columns of $K_{ X}^h$ are updated within the subspace spanned by the columns of $K_{ X}^h$ at initialization.
Thus, the preservation of condition (iii) is proved.

\paragraph{Preservation of condition (iv).}
Note that $\dot Q_{ X}^h = - d^{-1/2} K^h A_{:, X}^h = - d^{-1/2} K_{ X}^h A_{X, X}^h$, where the last equality holds since $A_{Y, X}^h = 0$. Hence, $\col(Q_{ X}^h)$ remains a subset of $\col(K_{ X}^h)$ given that $\col(K_{ X}^h)$ is unchanged under the gradient flow. 
\end{proof}

\paragraph{$V_{ X}^h$, $K_{ Y}^h$ and $Q_{ Y}^h$ are fixed at initialization.}
Following from \eqref{eq: dynamics of V^h-1} and \eqref{eq: dynamics of K^h-1}, we have that $V_{ X}^h$ and $K_{ Y}^h$ are fixed at initialization. 
It remains to show that $Q_{ Y}^h$ is also fixed at initialization.
We note that
\begin{align*}
    \dot Q_{ Y}^h = - \frac 1 {\sqrt{d}} K^h A_{:, Y}^h = 0, \quad \dot Q_{ X}^h = - \frac 1 {\sqrt{d}} K^h A_{:, X}^h = - \frac 1 {\sqrt{d}} K_{ X}^h A_{X, X}^h.
\end{align*}
Therefore, $Q_{ Y}^h$ is also fixed at initialization.




\subsection{Effective Order $\kappa$}
\Siyu{to be polished.}
Suppose $f=\prod_{i=1}^{n} \KK_{a_{i} b_{i}} \prod_{j=1}^{m} p_{c_{j}}$ is a polynomial of $p$ and $\KK$.
The effective order $\kappa$ of $f$ is defined as
$$
\kappa(f)=\underbrace{\cD(f)}_{\text{degree}=n+m}-\underbrace{\cC(f)}_{\# \text { of connected components }}, 
$$
where $\cD(f)$ is the degree of $f$ and $\cC(f)$ is the number of connected components of the graph $\cG$ associated with $f$. Here, $\cG$ is an undirected graph defined in the following way:
\begin{definition}[Associated graph for polynomials]
    For a polynomial $f$ of the form 
    $$f=\prod_{i=1}^{n} \KK_{a_{i} b_{i}} \prod_{j=1}^{m} p_{c_{j}},$$ 
    we define the associated graph $\cG$ as an undirected graph
    with nodes 
    $$V=\left\{v \mid v \in\left\{a_{i}\right\}_{i=1}^{n} \cup\left\{b_{i}\right\}_{i=1}^{n} \cup\left\{c_{j}\right\}_{j=1}^{m}\right\}$$ 
    and edges 
    $$E=\left\{\left(v, v^{\prime}\right) \in V^{2} \mid\left(v, v^{\prime}\right) \in\left\{\left(a_{i}, b_{i}\right)\right\}_{i=1}^{n}\right\}.$$
\end{definition}
Note that we allow the existence of self-loop in $\cG$ when $a_i=b_i$ for some $i\in[n]$. 
Intuitively, the effective order $\kappa$ measures the degree of $f$ in terms of $L^{-1}$. 
To see this, we consider a uniform probability $p_i = L^{-1}$ and $\KK_{ij} = L^{-1}\delta_{ij} - L^2 \approx L^{-1} \delta_{ij}$ for all $i, j\in[L]$.
By definition, the connected components in $\cG$ are connected by $\delta_{ij}$ in $\KK_{ij}$. 
Therefore, the number of free indices is actually equal to the number of connected components in $\cG$.
Since summing over each free index will add a factor of $L$, we subtract the number of connected components from the degree of $f$ to obtain the effective order $\kappa$.
It is easy to check that the following property holds, which will be useful in the sequel,
$$
\kappa\big(f\cdot \|p\|_{a}^{b}\big)=(\cD(f)+b)-\left(\cC(f)+\frac{b}{a}\right)=\kappa(f)+(a-1) \frac{b}{a}, \quad \text{where}\quad b \equiv 0 \mod a.
$$


\subsection{Dynamics of $O^h, V^h$.}
Recall from \eqref{eq: B^h-1} that
\begin{align}
    B^h &= \sum_{h'=1}^H O^{h'} V^{h'} \EE\begin{pmatrix}
        X p^{h'}(p^h)^\top X^\top & X p^{h'}(p^h)^\top X^\top \beta \notag\\
        \beta^\top X p^{h'}(p^h)^\top X^\top & \beta^\top X p^{h'}(p^h)^\top X^\top \beta + \varepsilon p^{h'}(p^h)^\top \varepsilon^\top
    \end{pmatrix} \notag\\
    &\qquad
    - \EE\left[
        \beta^\top x_q (p^h)^\top X^\top \begin{pmatrix} I_{d_x} , \beta \end{pmatrix}
    \right] 
    % \bluetag{$\varepsilon\indep (p^h, \beta, x_q)$} 
    \notag\\
    & = \sum_{h'=1}^H \EE\begin{pmatrix}
        \underbrace{O^{h'} V_{ X}^{h'}X p^{h'}(p^h)^\top X^\top}_{\ds =0}, & 
        O^{h'} V_{ Y}^{h'} \underbrace{\left(\beta^\top X p^{h'}(p^h)^\top X^\top \beta + \varepsilon p^{h'}(p^h)^\top \varepsilon^\top \right)}_{\numberlabel{1}}
    \end{pmatrix} 
    % \bluetag{$\EE[\beta]=0, \beta\indep (X, p^h)$}
    \notag\\
    &\qquad
    -
         \begin{pmatrix} 0 , & \underbrace{\EE\left[\beta^\top x_q (p^h)^\top X^\top\beta\right]}_{\numberlabel{2}} \end{pmatrix} , 
    \label{eq: B^h-2}
\end{align}
Next, we consider the two terms $\numberlabel{1}$ and $\numberlabel{2}$ separately.

\paragraph{Term $\numberlabel{1}$:}
Since the entries in the key and query weights that corresponds to the position of $y$ is zero, we also denote by $K^h$ and $Q^h$ the sub-matrix that corresponds to the position of $x$ for simplicity.
In the sequel, we let $W^h = (K^h)^\top Q^h/\sqrt d$. We evaluate $\EE[
    X p^{h'} (p^h)^\top X^\top
]$ as follows
\begin{align*}
    \EE\left[
        X p^{h'} (p^h)^\top X^\top
    \right]
    &= \sum_{l'} \EE\left[
        \nabla_{l'} \left(
            p_{l'}^{h'} (p^h)^\top X^\top
        \right)
    \right] \cdot \sigma_x^2
    \bluetag{Stein's lemma} \\
    % decompose the gradient
    &= \sum_{l'} \EE\left[
        \left(
            \nabla_{l'} p_{l'}^{h'} (p^h)^\top + p_{l'}^{h'} \nabla_{l'} (p^h)^\top
        \right) X^\top + p_{l'}^{h'} p_{l'}^h I
    \right] \cdot \sigma_x^2\\
    % use the stein's lemma again
    & = \sum_{l', l} \EE\left[
        \nabla_{l'} p_{l'}^{h'} \nabla_l^\top p_l^h + p_l^h \nabla_{l', l} p_{l'}^{h'} +  \nabla_{l'} p_l^h \nabla_{l}^\top p_{l'}^{h'}+ p_{l'}^{h'} \nabla_{l', l} p_l^h
    \right] \sigma_x^4 \\
    &\autoquad{2} + \sum_{l'} \EE\left[p_{l'}^{h'} p_{l'}^h\right] I \sigma_x^2
    \bluetag{Stein's lemma}, 
\end{align*}
where we denote by $\nabla_{l}(\cdot) = \nabla_{x_l}(\cdot)$ for simplicity. Here, we use the Stein's lemma twice to get rid of the in-context token $x_l$. 
We can further simplify the term as
\begin{align}
    &\EE\left[
        X p^{h'} (p^h)^\top X^\top
    \right] \notag\\
    &\quad = \sum_{l', l} \EE\left[
        W^{h'} x_q x_q^\top (W^h)^\top \KK_{l',l'}^{h'} \KK_{l, l}^h + W^h x_q x_q^\top (W^{h'})^\top \KK_{l',l}^{h} \KK_{l, l'}^{h'}
    \right] \sigma_x^4 \notag\\
    &\autoquad{3} + \sum_{l', l} \EE\left[
        W^{h'} x_q x_q^\top (W^{h'})^\top p_l^h \KK_{l', l}^{h'} (1 - 2 p_{l'}^{h'}) + W^h x_q x_q^\top (W^{h})^\top p_{l'}^{h'} \KK_{l', l}^{h} (1 - 2 p_l^h)
    \right] \sigma_x^4 \notag\\
    &\autoquad{3} + \sum_{l'} \EE\left[p_{l'}^{h'} p_{l'}^h\right] I_{d_x} \sigma_x^2 \notag\\ 
    & \quad = \sigma_x^4 \EE\left[
        W^{h'} x_q x_q^\top (W^h)^\top \left(1 - \norm{p^{h'}}_2^2\right) \left(1 - \norm{p^{h}}_2^2\right)
    \right] + \sigma_x^2 \EE[(p^{h'})^\top p^h] I_{d_x} \notag\\
    & \autoquad{3} + \sigma_x^4 \EE\left[
        W^h x_q x_q^\top (W^{h'})^\top \left( (p^{h})^\top p^{h'} - \sum_{l} p^{h}_l (p^{h'}_l)^2 - \sum_{l} p^{h'}_l (p^{h}_l)^2 + ((p^{h})^\top p^{h'})^2 \right) 
    \right] \notag\\
    & \autoquad{3} -2  \sigma_x^4 \EE\left[
        W^{h'} x_q x_q^\top (W^{h'})^\top \left( \sum_l p_l^{h} (p_l^{h'})^2 - (p^{h})^\top p^{h'} \norm{p^{h'}}_2^2\right)
    \right]\notag\\
    & \autoquad{3} -2  \sigma_x^4 \EE\left[
        W^{h} x_q x_q^\top (W^{h})^\top \left( \sum_l p_l^{h'} (p_l^{h})^2 - (p^{h'})^\top p^{h} \norm{p^{h}}_2^2\right)
    \right].
    \label{eq:grad-1}
\end{align}
where we use the following basic facts about the gradient of softmax probability
\begin{align*}
    \partial_l p_{l'} = \KK_{l, l'}, \quad \partial_{l', l}^2 p_{l} = \KK_{l', l}(1 - 2 p_l) , \quad \text{where}\quad \KK = \diag(p) - p p^\top.
\end{align*}
Here, we use $\partial_l(\cdot) = \partial_{s_l}(\cdot)$ to denote the derivative with respect to the softmax score and to distinguish from the previous notation $\nabla_l(\cdot) = \nabla_{x_l}(\cdot)$.
For $h'=h$, we have
\begin{align*}
    &\EE\left[
        X p^{h} (p^h)^\top X^\top
    \right] \\
    &\autoquad{1} = \sum_{l', l} \EE\left[
        W^{h} x_q x_q^\top (W^h)^\top 
        \left(\KK_{l',l'}^{h} \KK_{l, l}^h + \KK_{l',l}^{h} \KK_{l, l'}^{h} 
        + p_l^h \KK_{l', l}^{h} (1 - 2 p_{l'}^{h}) + p_{l'}^{h} \KK_{l', l}^{h} (1 - 2 p_l^h) \right)
    \right] \sigma_x^4\\
    &\autoquad{3} + \sum_{l'} \EE\left[p_{l'}^{h} p_{l'}^h\right] I \sigma_x^2\\
    &\autoquad{1} = \EE\left[
        W^{h} x_q x_q^\top (W^h)^\top 
        \left( \trace[\KK^h]^2 + \trace[\KK^h (\KK^h)^\top] - 4 \trace[p^h (p^h)^\top \KK^h]\right)
    \right] \sigma_x^4 + \sigma_x^2\EE\norm{p^h}^2 \cdot I_{d_x} \\
    &\autoquad{1} = \EE\left[
        W^{h} x_q x_q^\top (W^h)^\top 
        \left( 1 - \norm{p^h}_2^2 - 6 \norm{p^h}_3^3 + 6 \norm{p^h}_2^4\right)
        \right] \sigma_x^4 + \sigma_x^2\EE\norm{p^h}^2 \cdot I_{d_x}.
\end{align*}
In the same manner, we have for the noise term that
\begin{align*}
    \EE\left[\varepsilon p^{h'} (p^h)^\top \varepsilon^\top\right] 
    &=  \sigma_\varepsilon^2 \EE[(p^{h'})^\top p^h] \cdot I_{d_y} \cdot \ind(h'\neq h) + \sigma_\varepsilon^2\EE\norm{p^h}_2^2 \cdot I_{d_y} \cdot \ind(h'=h).
    % \\
    % &= \frac 1 L \sigma_\varepsilon^2 I_{d_y} \ind(h'\neq h) + \sigma_\varepsilon^2 \EE_{\epsilon\sim\cN(0, I_d)}\left[
        % \phi_L^2\left(\sigma_x^2\sqrt{\sum_{m=1}^d (\lambda_m^h)^2 \epsilon_m^2}\right)
    % \right] \cdot I_{d_y} \cdot \ind(h'=h)
\end{align*}

\textcolor{cyan}
{
To eliminate the cross-head interference, we notice the uncoupling property that $\langle W^h z, W^{h'} z\rangle = 0$ for all $z\in\RR^{d_x + d_y}$ and $h\neq h'$.
Two nice things are implied from this property. 
\begin{itemize}
    \item First, we have $W^h x_q x_q^\top (W^h)^\top$ for all $h\neq h'$.
    \item Second, $x_l^\top W^h x_q \indep x_{l'}^\top W^{h'} x_q$ for all $h\neq h'$ and $l, l'\in[L]$.
\end{itemize}
In addition, the second property here implies $p^h \indep p^{h'}$ for $h\neq h'$. 
Let us consider $h\neq h'$ for now. The first two terms in \eqref{eq:grad-1} cancel out by the first argument above. For the 3rd term, we have by $p^h \indep p^{h'}$ that
\begin{align*}
    \sum_{l', l} \EE\left[
        p_l^h \KK_{l', l}^{h'} (1 - 2 p_{l'}^{h'}) 
    \right]
    = \sum_{l', l} \EE\left[\EE[p_l^h\given x_q] \cdot \EE[
        \KK_{l', l}^{h'} (1 - 2 p_{l'}^{h'}) \given x_q
    ]\right] = \frac 1 L \sum_{l'} \EE\left[ \sum_{l}
        \KK_{l', l}^{h'} (1 - 2 p_{l'}^{h'})
    \right] = 0, 
\end{align*}
where we use the fact that $\EE[p_l^h|x_q] = 1/L$ and that the all one vector $\vone$ always lies in the null space of $\KK$. Therefore, the 3rd and 4th terms are also $0$.
The last term gives 
\begin{align*}
    \sum_{l'} \EE[p_{l'}^{h'} p_{l'}^h] I \sigma_x^2
    = \sum_{l'} \EE\left[\EE[p_{l'}^{h'}\given x_q] \EE[p_{l'}^h\given x_q]\right] I \sigma_x^2 = \frac 1 {L} I \sigma_x^2.\quad h\neq h'.
\end{align*}
}


\paragraph{Term $\numberlabel{2}$:}
The technique used here is similar to the previous one. We have
\begin{align*}
    \EE\left[
        x_q (p^h)^\top X^\top
    \right]
    &= \sigma_x^2 \sum_{l} \EE\left[
        x_q \nabla_l^\top p_l^h \right] \bluetag{Stein's lemma}\\
    &= \sigma_x^2 \sum_{l} \EE\left[
        x_q x_q^\top (W^h)^\top \KK_{l,l}^h \right] \notag\\
    &= \sigma_x^2 \EE\left[
        x_q x_q^\top (W^h)^\top (1 - \norm{p^h}_2^2) \right].
\end{align*}

\paragraph{Summary for $B^h$.}
In the sequel, we split $B^h$ into two parts, i.e., $B^h = (B_X^h, B_Y^h)$. Since we already have $B_X^h=0$, we only need to consider $B_Y^h$ as 
% For $B_X^h$, we have according to \eqref{eq: B^h-2} that
% \begin{align*}
%     B_X^h &= \sum_{h'=1}^H O^{h'} V_{ X}^{h'} \EE\left[X p^{h'}(p^h)^\top X^\top\right]\\
%         & = \sum_{h'=1}^H O^{h'} V_{ X}^{h'} 
%     \Bigg( 
%     {\color{magenta}
%         \sigma_x^4 \EE\left[
%         W^{h'} x_q x_q^\top (W^h)^\top \left(1 - \norm{p^{h'}}_2^2\right) \left(1 - \norm{p^{h}}_2^2\right) \right] + \sigma_x^2 \EE[(p^{h'})^\top p^h] I_{d_x}
%      } \notag\\
%     & \autoquad{3} + \sigma_x^4 \EE\left[
%         W^h x_q x_q^\top (W^{h'})^\top \left( (p^{h})^\top p^{h'} - \sum_{l} p^{h}_l (p^{h'}_l)^2 - \sum_{l} p^{h'}_l (p^{h}_l)^2 + ((p^{h})^\top p^{h'})^2 \right) 
%     \right] \notag\\
%     & \autoquad{3} -2  \sigma_x^4 \EE\left[
%         W^{h'} x_q x_q^\top (W^{h'})^\top \left( \sum_l p_l^{h} (p_l^{h'})^2 - (p^{h})^\top p^{h'} \norm{p^{h'}}_2^2\right)
%     \right]\notag\\
%     & \autoquad{3} -2  \sigma_x^4 \EE\left[
%         W^{h} x_q x_q^\top (W^{h})^\top \left( \sum_l p_l^{h'} (p_l^{h})^2 - (p^{h'})^\top p^{h} \norm{p^{h}}_2^2\right)
%     \right] \Bigg).
% \end{align*}
% For $B_Y^h$, we have
\begin{align*}
    B_Y^h & = \sum_{h'=1}^H O^{h'} V_{ Y}^{h'} \left[\beta^\top X p^{h'}(p^h)^\top X^\top \beta + \varepsilon p^{h'}(p^h)^\top \varepsilon^\top \right] - \EE\left[\beta^\top x_q (p^h)^\top X^\top \beta\right] \notag\\
    & = \sum_{h'=1}^H O^{h'} V_{ Y}^{h'} 
    \Bigg( 
    {\color{magenta}
        \sigma_x^4 \EE\left[
        \beta^\top W^{h'} x_q x_q^\top (W^h)^\top \beta \left(1 - \norm{p^{h'}}_2^2\right) \left(1 - \norm{p^{h}}_2^2\right) \right] + \left(\sigma_x^2  \EE[\beta^\top \beta] + \sigma_\varepsilon^2 I_{d_y}\right)\EE[(p^{h'})^\top p^h] 
     } \notag\\
    &\autoquad{3} + \sigma_x^4 \EE\left[
        \beta^\top W^h x_q x_q^\top (W^{h'})^\top\beta \left( {\color{magenta}(p^{h})^\top p^{h'}} - \sum_{l} p^{h}_l (p^{h'}_l)^2 - \sum_{l} p^{h'}_l (p^{h}_l)^2 + ((p^{h})^\top p^{h'})^2 \right) 
    \right] \notag\\
    & \autoquad{3} -2  \sigma_x^4 \EE\left[
        \beta^\top W^{h'} x_q x_q^\top (W^{h'})^\top\beta \left( \sum_l p_l^{h} (p_l^{h'})^2 - (p^{h})^\top p^{h'} \norm{p^{h'}}_2^2\right)
    \right]\notag\\
    & \autoquad{3} -2  \sigma_x^4 \EE\left[
        \beta^\top W^{h} x_q x_q^\top (W^{h})^\top \beta \left( \sum_l p_l^{h'} (p_l^{h})^2 - (p^{h'})^\top p^{h} \norm{p^{h}}_2^2\right)
    \right]\Bigg) \notag\\
    & \autoquad{3} {\color{magenta}
        - \sigma_x^2 \EE\left[
        \beta^\top x_q x_q^\top (W^h)^\top \beta (1 - \norm{p^h}_2^2) \right]
    }.
\end{align*}
We also have approximations for $B_Y^h$ as 
\begin{align}
    B_Y^h 
    &\approx \sum_{h'=1}^H  O^{h'} V_{ Y}^{h'} \Biggl( \left(\frac{\sigma_x^2}{d_x d_y}
    \cdot  R_\beta^\top \cT^\top(L_\beta^\top L_\beta) R_\beta + \sigma_\varepsilon^2 I_{d_y}\right)\cdot \EE[(p^{h'})^\top p^h] \notag\\
    &\autoquad{2} + \frac{\sigma_x^4 }{d_x d_y}\cdot
    \EE\left[R_\beta^\top \cT^\top\bigl(L_\beta^\top W^{h'} x_q x_q^\top (W^h)^\top L_\beta\bigr) R_\beta \cdot \left(1- \norm{p^h}_2^2 - \norm{p^{h'}}_2^2 + (p^h)^\top p^{h'}\right)\right]
    \Biggr) \notag\\
    &\autoquad{2} - \frac{\sigma_x^2}{d_x d_y} \cdot \EE\left[R_\beta^\top \cT^\top\bigl(L_\beta^\top x_q x_q^\top (W^h)^\top L_\beta\bigr) R_\beta \cdot (1-\norm{p^h}_2^2) \right], \label{eq: B_Y^h-approx}
\end{align}
where we denote by $\cT^\top(M) = \diag^{-1}(\tilde G^\top \diag(M))$ with $\tilde G$ being the variance matrix for each element of $G$. Note that $\cT^\top(\cdot)$ always gives a diagonal matrix.
% {\color{cyan}
% In particular, when the decoupling property holds, we can simplify the above expression as
% \begin{align*}
%     B_Y^h &= O^{h} V_{ Y}^{h} \left(\EE\left[
%         \beta^\top W^{h} x_q x_q^\top (W^h)^\top \beta
%         \left( 1 - \norm{p^h}_2^2 - 6 \norm{p^h}_3^3 + 6 \norm{p^h}_2^4\right)
%         \right] \sigma_x^4 + \EE\norm{p^h}^2 \cdot (\sigma_x^2\EE[\beta^\top \beta] + \sigma_\varepsilon^2 I_{d_y}) \right) \\
%     &\autoquad{2} - \sigma_x^2 \EE\left[
%         \beta^\top x_q x_q^\top (W^h)^\top  \beta (1-\norm{p^h}_2^2)
%     \right]  + \sum_{h'\neq h} O^{h'} V_{ Y}^{h'} \cdot \frac 1 L \left(\sigma_x^2 \EE[\beta^\top \beta ] + \sigma_\varepsilon^2 I_{d_y}\right)
% \end{align*}
% }



\subsection{Dynamics of $Q^h, K^h$.}
Recall from \eqref{eq: A^h-1} that we only need to characterize $A_{X, X}^h$ given by
\begin{align*}
    A_X^h &= \EE\left[ X \KK^h X^\top \beta  (U_Y^h)^\top \left( \sum_{h'} U_Y^{h'} \beta^\top X p^{h'} - \beta^\top x_q \right) x_q^\top \right] + \sum_{h'}\EE\left[X \KK^h  \varepsilon^\top
    (U_Y^h)^\top U_Y^{h'}\varepsilon
    p^{h'} x_q^\top\right].
\end{align*}
In the following, we denote by $p$, $\KK$ and $W$ the attention probability, attention kernel and attention weights for head $h$, and by $q$, $\QQ$ and $Q$ the correspondences for head $h'$, respectively.
Since the attention score does not depend on $Y$, we also simplify the notation by letting $W$ equal to $W_{X, X}$ and $Q$ equal to $Q_{X, X}$ when there is no ambiguity.
We first consider the following tensor with third moment of $X$. 
\begin{align*}
& \sum_{i, j, k} \mathbb{E}\left[\mathbb{K}_{i j} q_{k} x_{i} \otimes x_{j} \otimes x_{k}\right] \\
& \quad =\sigma_{x}^{2} \sum_{i, j, k} \mathbb{E}\left[\nabla_{x_{i}}\left(\mathbb{K}_{i j} q_{k}\right) \otimes x_{j} \otimes x_{k}+\mathbb{K}_{i j} q_{k}\left(\delta_{i j} I^{12} \otimes x_{k}+\delta_{i k}\left(I^{13} \otimes x_{j}\right)^{\top_{132}}\right)\right] \\
& \quad =
    \underbrace{
        \sigma_{x}^{2} \sum_{i, j, k} \mathbb{E}\left[\nabla_{x_{i}}\left(\mathbb{K}_{i j} q_{k}\right) \otimes x_{j} \otimes x_{k}\right]
    }_{\dstext{(a)}}
    +\underbrace{
        \delta_{x}^{2} \sum_{j, k} \mathbb{E}\left[\mathbb{K}_{j j} q_{k} I^{12} \otimes x_{k}+\mathbb{K}_{k j} q_{k}\left(I^{13} \otimes x_{j}\right)^{\top_{132}}\right] 
    }_{\dstext{(b)}}, 
\end{align*}
where in the first equality, we invoke the Stein's lemma. Here, we use superscript in $I^{12}$ to remind ourselves that this identity matrix comes from $\nabla_{x_i} x_j^\top$ and so on for $I^{13}$ and $I^{23}$. We also denote by $\top_{132}$ the transpose operation that transposes the second and third dimensions of a tensor.
For term (a), we have by the Stein's lemma that
$$
\begin{aligned}
\dstext{(a)}& =\sigma_{x}^{2} \sum_{i, j, k} \mathbb{E}\left[\nabla_{x_{i}}\left(\mathbb{K}_{i j} q_{k}\right) \otimes x_{j} \otimes x_{k}\right] \\
& =\sigma_{x}^{4} \sum_{i, j, k} \mathbb{E}\left[\left(\nabla_{x_{i}} \otimes \nabla_{x_{j}}\right)\left(\mathbb{K}_{i j} q_{k}\right) \otimes x_{k}+\delta_{j k} \nabla_{x_{i}}\left(\mathbb{K}_{i j} q_{k}\right) \otimes I^{23}\right] \\
& =\underbrace{
        \sigma_{x}^{4} \sum_{i, j, k} \mathbb{E}\left[\left(\nabla_{x_{i}} \otimes \nabla_{x_{j}}\right)\left(\KK_{i j} q_{k}\right) \otimes x_{k}\right]
    }_{\dstext{(a.1)}}
    +\underbrace{\sigma_{x}^{4} \sum_{i, j} \mathbb{E}\left[\nabla_{x_{i}}\left(\KK_{i j} q_{j}\right) \otimes I^{23}\right]}_{\dstext{(a.2)}}.
\end{aligned}
$$
For (a.1), we further have
$$
\begin{aligned}
\dstext{(a.1)} 
& =\sigma_{x}^{4} \sum_{i, j, k} \mathbb{E}\left[\left(\nabla_{x_{i}} \otimes \nabla_{x_{j}}\right)\left(\KK_{i j} q_{k}\right) \otimes x_{k}\right] \\
& =\sigma_{x}^{6} \sum_{i, j, k} \mathbb{E}\left[\left(\nabla_{x_{i}} \otimes \nabla_{x_{j}} \otimes \nabla_{x_{k}}\right)\left(\mathbb{K}_{i j} q_{k}\right)\right] 
\eqdef \dstext{(a.1)}^*.
\end{aligned}
$$
For $\dstext{(a.2)}$, we have
$$
\dstext{(a.2)}=\sigma_{x}^{4} \sum_{i, j} \mathbb{E}\left[\nabla_{x_{i}}\left(\mathbb{K}_{i j} q_{j}\right) \otimes I^{23}\right]=\sigma_{x}^{4} \sum_{i} \mathbb{E}\left[\nabla_{x_{i}}\big(p_{i}(q_{i}-p^{\top} q)\big) \otimes I^{23}\right]=\dstext{(a.2)}^{*}.
$$
For (b), we also have
$$
\begin{aligned}
\dstext{(b)} & =\sigma_{x}^{2} \sum_{j, k} \mathbb{E}\left[\mathbb{K}_{j j} q_{k} I^{12} \otimes x_{k}+\mathbb{K}_{k j} q_{k}\left(I^{13} \otimes x_{j}\right)^{\top_{132}}\right] \\
& =\sigma_{x}^{4} \sum_{j, k} \mathbb{E}\left[I^{12} { \otimes} \nabla_{x_{k}}\left(\mathbb{K}_{j j} q_{k}\right)\right]+\sigma_{x}^{4} \sum_{j, k} \mathbb{E}\left[\left(I^{13} \otimes \nabla_{x_{j}}\left(\mathbb{K}_{k j} q_{k}\right)\right)^{\top_{132}}\right] \\
& =\underbrace{
        \sigma_{x}^{4} \sum_{k} \mathbb{E}\left[I^{12} \otimes \nabla_{x_{k}}\left(\left(1-\|p\|_{2}^{2}\right) q_{k}\right)\right]
    }_{\dstext{(b.1)}}
    +\underbrace{
        \sigma_{x}^{4} \sum_{j} \mathbb{E}\left[\left(I^{13} \otimes \nabla_{x_{j}}\big(p_{j} (q_{j}-p^{\top} q )\big)\right)^{\top_{132}}\right]
    }_{\dstext{(b.2)}}.
\end{aligned}
$$
For $\dstext{(a.1)}^{*}$, we claim that the following holds:
\begin{center}
    \begin{tabular}{l@{\hspace{1cm}}l}
        \hline
        \hline
        \textbf{Terms in the split of $\dstext{(a.1)}^*$} & \textbf{Coefficient} \\
        \hline
        $\sum_{i, j, k} W x_q \otimes W x_q \otimes W x_{q} \cdot \partial_{i j k}^{3}\left(\KK_{i j}\right) q_{k}$ & $\kappa \geqslant 2$ \\
        $\sum_{i, j, k} {W'} x_{q} \otimes W x_q \otimes W x_{q} \cdot \partial_{j k}^{2}\left(\KK_{i j}\right) \partial_{i}\left(q_{k}\right)$ & $\kappa \geqslant 2$ \\
        $\sum_{i, j, k} W x_{q} \otimes {W'} x_{q} \otimes W x_{q} \cdot \partial_{i k}^{2}\left(\KK_{i j}\right) \partial_{j}\left(q_{k}\right)$ & $\kappa \geqslant 2$ \\
        $\sum_{i, j, k} W x_q \otimes W x_q \otimes {W'} x_q \cdot \partial_{i j}^{2}\left(\KK_{i j}\right) \partial_{k}\left(q_{k}\right)$ & $-2\|p\|_{2}^{2}$ \\
        $\sum_{i, j, k} {W'} x_{q} \otimes {W'} x_q \otimes W x_{q} \cdot \partial_{k}\left(\KK_{i j}\right) \partial_{i j}^{2}\left(q_{k}\right)$ & $p^{\top} q$ \\
        $\sum_{i, j, k} {W'} x_{q} \otimes W x_{q} \otimes {W'} x_q \cdot \partial_{j}\left(\mathbb{K}_{i j}\right) \partial_{i k}^{2}\left(q_{k}\right)$ & $\kappa \geqslant 2$ \\
        $\sum_{i, j, k} W x_{q} \otimes {W'} x_{q} \otimes {W'} x_{q}\cdot \partial_{i}\left(\KK_{i j}\right) \partial_{j k}^{2}\left(q_{k}\right)$ & $\kappa \geqslant 2$ \\
        $\sum_{i, j, k} {W'} x_{q} \otimes {W'} x_{q} \otimes {W'} x_{q} \cdot \KK_{i j} \partial_{i j k}^{3}\left(q_{k}\right)$ & $\kappa \geqslant 2$ \\
        \hline
        \hline
    \end{tabular}
\end{center}
Therefore, 
$$
\begin{aligned}
\dstext{(a.1)}^{*} & =\sigma_{x}^{b} \sum_{i, j, k} \mathbb{E}\left[\left(\nabla_{x_{i}} \otimes \nabla_{x j} \otimes \nabla_{x_{k}}\right)\left(\mathbb{K}_{i j} q_{k}\right)\right] \\
& = \sigma_{x}^{6} \mathbb{E}\left[-2\|p\|_{2}^{2} W x_q \otimes W x_{q} \otimes {W'} x_q+p^{\top} q {W'} x_{q} \otimes {W'} x_q \otimes W x_q\right] \\
& \qquad + \sigma_{x}^6 \EE\left[
    \sum_{(P_1, P_2, P_3)\in\{W, {W'}\}^{3}\backslash \{(W, W, {W'}), ({W'}, {W'}, W)\}} \Phi_2(p, q) \cdot P_1 x_q \otimes P_2 x_q \otimes P_3 x_q 
\right],
\end{aligned}
$$
where $\Phi_2(p, q)$ represents coefficients with $\kappa\geqslant 2$. 
For easy of notation, we will use \say{$\approx$} to ignore the terms with $\kappa\geqslant 2$ in the following.
For the remaining terms, we follow the same procedure and obtain
\begin{center}
    \begin{tabular}{p{4.5cm}@{\hspace{1cm}} p{9cm}}
        \hline
        \hline
        \textbf{Terms in $\sum_{i,j,k}\EE[\KK_{ij}q_k x_i \otimes x_j\otimes x_k]$} & \textbf{Dominating term} \\
        \hline
        $\dstext{(a.1)}^*$ & $\sigma_x^6 \EE[-2\|p\|_2^2 W x_q \otimes W x_q \otimes {W'} x_q + p^\top q {W'} x_q \otimes {W'} x_q \otimes W x_q]$ \\
        $\dstext{(a.2)}^*$ & $\sigma_x^4 \EE[p^\top q \cdot {W'} x_q \otimes I^{23}]$ \\
        $\dstext{(b.1)}$ & $\sigma_x^4 \EE[(1 - \norm{p}_2^2 - \norm{q}_2^2) \cdot I^{12}\otimes {W'} x_q]$ \\
        $\dstext{(b.2)}$ & $\sigma_x^4 \EE[p^\top q \cdot (I^{13} \otimes {W'} x_q)^{\top_{132}}]$ \\
        \hline
    \end{tabular}
\end{center}
Therefore, we have
\begin{align*}
    \sum_{i,j,k} \EE\left[\KK_{ij}q_k x_i\otimes x_j\otimes x_k\right]
    &\approx \sigma_x^6 \EE\left[-2\|p\|_2^2 W x_q\otimes W x_q\otimes {W'} x_q + p^\top q {W'} x_q\otimes {W'} x_q\otimes W x_q\right]\\
    &\qquad + \sigma_x^4 \EE\left[p^\top q ({W'} x_q) \otimes I^{23}\right] + \sigma_x^4 \EE\left[p^\top q \left(I^{13} \otimes ({W'} x_q)\right)^{\top_{132}}\right]\\
    &\qquad + \sigma_x^4 \EE\left[\bigl(1-\norm{p}_2^2 - \norm{q}_2^2\bigr) I^{12}\otimes {W'} x_q\right].
\end{align*}
We next characterize
$$
\begin{aligned}
\sum_{i, j} \mathbb{E}\left[\mathbb{K}_{i j} x_{i} x_{j}^{\top}\right]
& =\sigma_{x}^{2} \cdot \sum_{i, j} \mathbb{E}\left[\nabla_{x_{i}}\left(\mathbb{K}_{i j}\right) x_{j}^{\top}+\delta_{i j} \mathbb{K}_{i j} I\right] \\
& =\sigma_{x}^{2} \sum_{i, j} \mathbb{E}\left[\mathbb{K}_{i j}\left(1-2 p_{i}\right) W x_{q} x_{j}^{\top}\right]+\sigma_{x}^{2}\left(1-\|p\|_{2}^{2}\right) I \\
& =\underbrace{\sigma_{x}^{2}(-2) \sum_{j} \mathbb{E}\left[\left(p_{j}^{2}-\|p \|_{2}^{2} p_{j}\right) W x_{q} x_{j}^{\top}\right]}_{\dstext{(c)}}+\sigma_{x}^{2}\left(1-\|p\|_{2}^{2}\right) I. 
\end{aligned}
$$
We use the same argument and have for (c) that
$$
\begin{aligned}
\dstext{(c)} & =-2 \sigma_{x}^{4} \sum_{j} \mathbb{E}\left[\left(2 p_{j} \mathbb{K}_{j j}-\mathbb{K}_{i j}\|p\|_{2}^{2}-p_{j} \cdot 2\left(p_{j}^{2}-\|p\|_{2}^{2} p_{j}\right)\right) W {x_q} x_{q}^{\top} W^{\top}\right] \\
& = -2 \sigma_{x}^{4} \mathbb{E}\left[(\|p\|_{2}^{2} + \Phi_2(p)) W x_{q} x_{q}^{\top} W^{\top}\right].
\end{aligned}
$$
Therefore,
$$
\begin{aligned}
\sum_{i, j} \mathbb{E}\left[\mathbb{K}_{i j} x_{i} x_{j}^{\top}\right] 
= -2 \sigma_{x}^{4} \mathbb{E}\left[(\|p\|_{2}^{2} + \Phi_2(p)) W x_{q} x_{q}^{\top} W^{\top}\right]+\sigma_{x}^{2}\left(1-\|p\|_{2}^{2}\right) I. 
\end{aligned}
$$
It remains to characterize the terms with noise. 
We first notice that
\begin{align*}
    \sum_{i, j, k} \mathbb{E}\left[\mathbb{K}_{i j} q_{k} x_{i} \otimes \varepsilon_{j} \otimes \varepsilon_{k}\right]  &=\sigma_{\varepsilon}^{2} \sum_{i, j} \mathbb{E}\left[\mathbb{K}_{i j} q_{j} x_{i} \otimes I_{d_{y}}\right] \\
    &  =\sigma_{\varepsilon}^{2} \sigma_{x}^{2} \sum_{i} \mathbb{E}\left[\nabla_{x_{i}}\left(p_{i} q_{i}-p_{i} p^{\top} q\right) \otimes I_{d_{y}}\right] \\
    &  =\sigma_{\varepsilon}^{2} \sigma_{x}^{2} \sum_{i} \mathbb{E}\left[\left(\mathbb{K}_{i i} q_{i}-\mathbb{K}_{i i} \bar{p}^{\top} q-\sum_{l} \mathbb{K}_{i l} q_{l} p_{i}\right) W {x_{q}} \otimes I_{d_{y}}\right] \\
    & \autoquad{2} +\sigma_{\varepsilon}^{2} \sigma_{x}^{2} \sum_{i} \mathbb{E}\left[\left(p_{i} \mathbb{Q}_{i i}-\sum_{l} p_{i} p_{l} \mathbb{Q}_{i l}\right) {W'} {x_{q}} \otimes I_{d_y}\right] \\
    & \approx \sigma_{\varepsilon}^{2} \sigma_{x}^{2} \mathbb{E}\left[p^{\top} q \cdot {W'} x_{q} \otimes I_{d y}\right]. 
\end{align*}
Similar result also holds for $\sum_{i, j, k} \mathbb{E}\left[\mathbb{K}_{i j} q_{k} \varepsilon_{i} \otimes x_{j} \otimes \varepsilon_{k}\right]$. For $\sum_{i, j, k} \mathbb{E}\left[\mathbb{K}_{i j} q_{k} \varepsilon_{i} \otimes \varepsilon_{j} \otimes x_{k}\right]$, we have
\begin{align*}
    \sum_{i, j, k} \mathbb{E}\left[\mathbb{K}_{i j} q_{k} \varepsilon_{i} \otimes \varepsilon_{j} \otimes x_{k}\right] 
    & =\sigma_{\varepsilon}^{2} \sum_{i, k} \mathbb{E}\left[\left(p_{i}-p_{i}^{2}\right) q_{k} I_{d_{y}} \otimes x_{k}\right] \\
    & =\sigma_{\varepsilon}^{2} \sigma_{x}^{2} \sum_{k} \mathbb{E}\left[I_{d y} \otimes \nabla_{x_{k}}\left(\left(1-\|p\|_{2}^{2}\right) q_{k}\right)\right] \\
    & =\sigma_{\varepsilon}^{2} \sigma_{x}^{2} \sum_{k}^{K} \mathbb{E}\left[I_{d y} \otimes\left(\mathbb{Q}_{k k}\left(1-\|p\|_{2}^{2}\right) {W'} x_{q}-q_{k} \sum_{l} 2 P_{l} \mathbb{K}_{l k} W x_{q}\right)\right] \\
    & \approx \sigma_{\varepsilon}^{2} \sigma_{x}^{2} \mathbb{E}\left[\left(1-\|q\|_{2}^{2}-\|p\|_{2}^{2}\right) I_{d y} \otimes {W'} {x_q}\right]
\end{align*}
We summarize the results in the following table:
\begin{center}
    \begin{tabular}{p{4.5cm}@{\hspace{1cm}} p{9cm}}
        \hline
        \hline
        \textbf{Terms} & \textbf{Dominating term} \\
        \hline
        $\sum_{i,j,k}\EE[\KK_{ij}q_k x_i \otimes \varepsilon_j \otimes \varepsilon_k]$ & $\sigma_{\varepsilon}^2 \sigma_x^2 \EE[p^\top q \cdot {W'} x_q \otimes I_{d_y}]$ \\
        $\sum_{i,j,k}\EE[\KK_{ij}q_k \varepsilon_i \otimes x_j \otimes \varepsilon_k]$ & $\sigma_{\varepsilon}^2 \sigma_x^2 \EE[p^\top q \cdot \left(I_{d_y} \otimes {W'} x_q\right)^{\top_{132}}]$ \\
        $\sum_{i,j,k}\EE[\KK_{ij}q_k \varepsilon_i \otimes \varepsilon_j \otimes x_k]$ & $\sigma_{\varepsilon}^2 \sigma_x^2 \EE[(1 - \norm{p}_2^2 - \norm{q}_2^2) \cdot I_{d_y} \otimes {W'} x_q]$ \\
        \hline
    \end{tabular}
\end{center}
The noise term in $A_{X, X}^{h, h'}$ is then given by 
\begin{align*}
    &\EE\left[
        \begin{pmatrix} 
            X \KK^h  \varepsilon^\top
            (U_Y^h)^\top U_Y^{h'}\varepsilon
            p^{h'} x_q^\top 
            \\
            \varepsilon \KK^h \varepsilon^\top (U_Y^h)^\top U_X^{h'} X p^{h'} x_q^\top + \varepsilon \KK^h X^\top (U_X^h)^\top U_Y^{h'} \varepsilon
            p^{h'} x_q^\top
        \end{pmatrix}
        \right] \\
    &\quad \approx \sigma_\varepsilon^2 \sigma_x^2 \EE\left[\begin{pmatrix}
        p^\top q \cdot \trace[(U_Y^h)^\top U_Y^{h'}] W^{h'} x_q x_q^\top \\
        (1- \norm{p}_2^2 - \norm{q}_2^2) \cdot (U_Y^h)^\top U_X^{h'} W^{h'} x_q x_q^\top + p^\top q \cdot (U_Y^{h'})^\top U_X^h W^{h'} x_q x_q^\top
    \end{pmatrix}\right].
\end{align*}
In summary, 
we can decompose $A_{X, X}^{h}$ as 
\begin{align}
    A_{X, X}^{h} = \sum_{h'=1}^H \left(A^{h, h'}_{X, X, \signal} + A^{h, h'}_{X, X, \noise} \right) + A_{X, X}^{h, 0},
    \label{eq: A_{X, X}^h-decompose} 
\end{align}
where we characterize the parts that corresponds to the position of $X$ as 
\begin{align}
    &A_{X, X, \signal}^{h, h'} \notag\\
    & \quad \approx \frac{1}{d_x d_y} \cdot \biggl(\sigma_x^4\EE\left[
        (p^h)^\top p^{h'}  \trace\left[L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top \right]  W^{h'} x_q x_q^\top \right]\notag\\
    &\autoquad{3} 
        + \sigma_x^4 \EE\Big[(1-\norm{p^h}_2^2 - \norm{p^{h'}}_2^2 + (p^h)^\top p^{h'}) L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top
       W^{h'} x_q x_q^\top
    \Big] \notag\\
    & \autoquad{3} + \sigma_x^6 \EE\Bigl[
        -2\norm{p^h}_2^2  W^h x_q x_q^\top (W^h)^\top    
        L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top W^{h'} x_q x_q^\top
    \Bigr] \notag\\
    & \autoquad{3} + \sigma_x^6 \EE\Bigl[
        (p^h)^\top p^{h'} W^{h'} x_q x_q^\top (W^{h'})^\top
        L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top W^{h} x_q x_q^\top
    \Bigr]\biggr)
    \label{eq: A_{X, X}^{h, h'}-signal}
\end{align}
where $\cT(M) = \diag^{-1}(\tilde G \diag(M))$ with $\tilde G$ being the variance matrix for each element of $G$.
Here, the approximation \say{$\approx$} comes from the fact that we ignore other possible combinations (either related to $W^h$ in the first two terms or $(P_1, P_2, P_3)\in\{W^h, W^{h'}\}^{3}\backslash \{(W^h, W^h, W^{h'}), (W^{h'}, W^{h'}, W^h)\}$ in the latter two terms) with $\kappa\geqslant 2$.
We also have for the noise term 
\begin{align}
    A^{h,h'}_{X, X,\noise} \approx - \sigma_\varepsilon^2 \sigma_x^2 \EE\left[
        (p^h)^\top p^{h'} \cdot \trace[(U_Y^h)^\top U_Y^{h'}] W^{h'} x_q x_q^\top
    \right],
    \label{eq: A_{X, X}^{h, h'}-noise}
\end{align}
where we also ignore the higher order term with $W^{h'}$ replaced by $W^h$.
Finally, we have the term that corresponds to $A^{h,0}$
\begin{align}
    A_{X, X}^{h, 0} = \frac{1}{d_x d_y}\cdot \EE\left[
        \left(-\sigma_x^2 (1 - \norm{p^h}_2^2)  +  2\sigma_x^4 (\norm{p^h}_2^2 + \Phi_2(p^h)) W^h x_q x_q^\top (W^h)^\top\right) L_\beta \cT\big(R_\beta (U_Y^h)^\top R_\beta^\top\big) L_\beta^\top x_q x_q^\top
    \right].
    \label{eq: A_{X, X}^{h, 0}}
\end{align}


\subsection{Equivalent Dynamics on the Eigenvalue Space}
In this subsection, we consider the projected dynamics on the eigen space.
We give the following definition on the alignment of the eigen spaces for $K, Q, V$ and $O$ with respect to $L_\beta$ and $R_\beta$.
\begin{definition}[Alignment Property]
    \label{def: alignment property}
    We say that a set of parameters $\{O^h, V^h, K^h, Q^h\}_{h=1}^H$ aligns under $(\varphi, \phi, v, u)$ if the following statement holds: 
    
    There exist sets of orthogonal unit vectors 
    $$\varphi=\{\varphi_1,\dots,\varphi_{d_y}\} \in \RR^{d_y}, \quad v_Y= \{v_{Y, 1},\dots,v_{Y, d_y}\}\in\RR^{D}, \quad v_X =\{v_{X, 1},\dots, v_{X, d_x}\}\in\RR^{D},$$ 
    where $v=\{v_{X}, v_Y\}$ and $v_{X,k}$ has the last $d_y$ entries being zero while $v_{Y, k}$ has the first $d_x$ entries being zero. 
    And there also exist sets of orthogonal vectors $\phi=\{\phi^h\}_{h\in[H]}, u=\{u^h\}_{h\in[H]}$ with
    $$\phi^h = \{\phi_1^h,\dots\phi_{d_y}^h\}\in\RR^{d},\quad u^h = \{u_{1}^h,\dots,u_{d_x}^h, \dots, u_{D}^h \}\in\RR^{d}, \quad \forall h\in [H], $$ 
    such that
    each vector's 2-norm is either $1$ or $0$. 
    With these eigen vectors, $O^h, V^h, K^h, Q^h$ admit the following decompositions
    \begin{gather} 
        O^h = \sum_{k=1}^{d_y} \lambda_{O,k}^h \varphi_k (\phi_k^h)^\top, \quad V^h = \underbrace{\sum_{k=1}^{d_y} \lambda_{V, k}^h \phi_k^h v_{Y, k}^\top}_{\ds V_{ Y}^h} + \underbrace{\sum_{m=1}^{d_x} \lambda_{V, d_y + m}^h \phi_{k+m}^h v_{X, m}^\top}_{\ds V_{ X}^h}, \notag\\
K^h = \underbrace{\sum_{k=1}^{d_x} \lambda_{K, k}^h u_{k}^h (v_{X, k})^\top}_{\ds K_{ X}^h} + \underbrace{\sum_{m=1}^{d_y} \lambda_{K, d_x+m}^h u_{d_x+m}^h (v_{Y, m})^\top}_{\ds K_{ Y}^h}, \notag\\
Q^h = \underbrace{\sum_{k=1}^{d_x} \lambda_{Q, k}^h u_{k}^h (v_{X, k})^\top}_{\ds Q_{ X}^h} + \underbrace{\sum_{m=1}^{d_y} \lambda_{Q, d_x+m}^h u_{d_x+m}^h (v_{Y, m})^\top}_{\ds Q_{ Y}^h}. \label{eq: aligned weight decomposition}
    \end{gather}
\end{definition}
We first have the observation that the alignment property implies the uncoupling property in \Cref{def:uncoupling X Y property}.
\begin{observation}\label{obs: alignment implies uncoupling}
    Suppose that a set of parameters $\{O^h, V^h, K^h, Q^h\}_{h=1}^H$ aligns under $(\varphi, \phi, v, u)$ as defined in \Cref{def: alignment property}.
    Then, the uncoupling property in \Cref{def:uncoupling X Y property} holds.
\end{observation}
We next characterize under what condition we can reduce the dynamics to only the eigenvalue space. 
\begin{proposition}
    \label{prop: dynamics on eigen space}
    Suppose that the initialization satisfies the alignment property with $(\varphi, \phi, v, u)$ as
     in \Cref{def: alignment property}. 
    If $v_X$ corresponds to the columns of $L_\beta$ and $v_Y$ corresponds to the rows of $R_\beta$, the dynamics can then be reduced to the eigenvalue space as an equivalent dynamics on $\lambda_{O}^h, \lambda_{V}^h, \lambda_{K}^h, \lambda_{Q}^h$ for all $h\in[H]$.
\end{proposition}
\begin{proof}
    By \Cref{obs: alignment implies uncoupling} and \Cref{prop: uncoupling dynamics}, we have that $V_{ X}$, $K_{ Y}$ and $Q_{ Y}$ will be fixed at initialization. The remaining dynamics are given by
    \begin{gather}
        \dot V_{ Y}^h = - (O^h)^\top B_Y^h,\quad \dot O^h = - B_Y^h V_{ Y}^h, \notag\\
        \dot K_{ X}^h = - \frac{1}{\sqrt d} Q_{ X}^h (A_{X, X}^h)^\top, \quad \dot Q_{ X}^h = - \frac{1}{\sqrt d} K_{ X}^h A_{X, X}^h,  \label{eq: uncoupled dynamics}
    \end{gather}
    where $B_Y^h$ is approximated by \eqref{eq: B_Y^h-approx} and $A_{X, X}^h$ is given by \eqref{eq: A_{X, X}^h-decompose} with each terms being approximated by \eqref{eq: A_{X, X}^{h, h'}-signal}, \eqref{eq: A_{X, X}^{h, h'}-noise} and \eqref{eq: A_{X, X}^{h, 0}}. 
    Our goal is to show that $B_Y^h$ and $A_{X, X}^h$ admit the following decompositions
    \begin{align*}
        B_Y^h = \sum_{k=1}^{d_y} \lambda_{B, k}^h \varphi_k (v_{Y, k})^\top, \quad A_{X, X}^h = \sum_{k=1}^{d_x} \lambda_{A, k}^h v_{X, k} (v_{X, k})^\top, 
    \end{align*}
    as it will imply that the dynamics are reduced to the eigenvalue space when plugged into \eqref{eq: uncoupled dynamics}.
    
    \paragraph{Decomposition of $B_Y^h$.}
    For completeness, we present \eqref{eq: B_Y^h-approx} here again:
    \begin{align*}
        B_Y^h 
    &\approx \sum_{h'=1}^H  O^{h'} V_{ Y}^{h'} \Biggl( \left(\frac{\sigma_x^2}{d_x d_y}
    \cdot  R_\beta^\top \cT^\top(L_\beta^\top L_\beta) R_\beta + \sigma_\varepsilon^2 I_{d_y}\right)\cdot \EE[(p^{h'})^\top p^h] \notag\\
    &\autoquad{2} + \frac{\sigma_x^4 }{d_x d_y}\cdot
    \EE\left[R_\beta^\top \cT^\top\bigl(L_\beta^\top W^{h'} x_q x_q^\top (W^h)^\top L_\beta\bigr) R_\beta \cdot \left(1- \norm{p^h}_2^2 - \norm{p^{h'}}_2^2 + (p^h)^\top p^{h'}\right)\right]
    \Biggr) \notag\\
    &\autoquad{2} - \frac{\sigma_x^2}{d_x d_y} \cdot \EE\left[R_\beta^\top \cT^\top\bigl(L_\beta^\top x_q x_q^\top (W^h)^\top L_\beta\bigr) R_\beta \cdot (1-\norm{p^h}_2^2) \right], 
    \end{align*}
    where the \say{$\approx$} only hides higher order coefficient with respect to $p^h$ and $p^{h'}$ and it does not affect our proof here. 
    Thus, it suffices to show that the following four terms can be decomposed onto rank one matrices $\{\varphi_k (v_{Y, k})^\top\}_{k\in[d_y]}$,
    \begin{gather*}
        O^{h'} V_{ Y}^{h'} R_\beta^\top \cT^\top(L_\beta^\top L_\beta) R_\beta, 
        \quad
        O^{h'} V_{ Y}^{h'} R_\beta^\top \cT^\top\bigl(L_\beta^\top W^{h'} x_q x_q^\top (W^h)^\top L_\beta\bigr) R_\beta, \\
        R_\beta^\top \cT^\top\bigl(L_\beta^\top x_q x_q^\top (W^h)^\top L_\beta\bigr) R_\beta,
        \quad
        O^{h'} V_{ Y}^{h'}
    \end{gather*} 
    Note that $\cT^\top(\cdot)$ always gives a diagonal matrix. Therefore, if we apply $\varphi_k$ to the left and $v_{Y, k'}$ to the right, only $k=k'$ gives nonzero results, given the decomposition of $O^h$ and $V_{ Y}^h$ in \eqref{eq: aligned weight decomposition} and the alignment between $R_\beta$ and $v_Y$. 
    Therefore, we prove that $B_Y^h$ admits the desired decomposition. 

    \paragraph{Decomposition of $A_{X, X}^h$.}
    We first present \eqref{eq: A_{X, X}^h-decompose} $A_{X, X}^{h} = \sum_{h'=1}^H \left(A^{h, h'}_{X, X, \signal} + A^{h, h'}_{X, X, \noise} \right) + A_{X, X}^{h, 0}$ with each terms being approximated by \eqref{eq: A_{X, X}^{h, h'}-signal}, \eqref{eq: A_{X, X}^{h, h'}-noise} and \eqref{eq: A_{X, X}^{h, 0}}:
    \begin{align*}
        &A_{X, X, \signal}^{h, h'} \notag\\
    & \quad \approx \frac{1}{d_x d_y} \cdot \biggl(\sigma_x^4\EE\left[
        (p^h)^\top p^{h'}  \trace\left[L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top \right]  W^{h'} x_q x_q^\top \right]\notag\\
    &\autoquad{3} 
        + \sigma_x^4 \EE\Big[(1-\norm{p^h}_2^2 - \norm{p^{h'}}_2^2 + (p^h)^\top p^{h'}) L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top
       W^{h'} x_q x_q^\top
    \Big] \notag\\
    & \autoquad{3} + \sigma_x^6 \EE\Bigl[
        -2\norm{p^h}_2^2  W^h x_q x_q^\top (W^h)^\top    
        L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top W^{h'} x_q x_q^\top
    \Bigr] \notag\\
    & \autoquad{3} + \sigma_x^6 \EE\Bigl[
        (p^h)^\top p^{h'} W^{h'} x_q x_q^\top (W^{h'})^\top
        L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top W^{h} x_q x_q^\top
    \Bigr]\biggr), \notag\\
    &A^{h,h'}_{X, X,\noise} \approx \sigma_\varepsilon^2 \sigma_x^2 \cdot \EE\left[
            (p^h)^\top p^{h'} \cdot \trace[(U_Y^h)^\top U_Y^{h'}] W^{h'} x_q x_q^\top\right], \notag\\
    &A_{X, X}^{h, 0} = \frac{1}{d_x d_y}\cdot \EE\left[
                \left(-\sigma_x^2 (1 - \norm{p^h}_2^2)  +  2\sigma_x^4 (\norm{p^h}_2^2 + \Phi_2(p^h)) W^h x_q x_q^\top (W^h)^\top\right) L_\beta \cT\big(R_\beta (U_Y^h)^\top R_\beta^\top\big) L_\beta^\top x_q x_q^\top
            \right]. 
    \end{align*}
    where $W^h$ is a simplification of $W_{X, X}^h$ and the \say{$\approx$} only hides higher order coefficient with respect to $p^h$ and $p^{h'}$. However, since $p^h$ and $p^{h'}$ are coupled with $x_q$ this time, we have to be more careful. 
    To this end, it suffices to show that the following terms can be decomposed onto rank one matrices $\{v_{X, k} (v_{X, k})^\top\}_{k\in[d_x]}$:
    \begin{gather*}
        \numberlabel{1}=\EE\left[
            f(p^h, p^{h'}) W^{h'} x_q x_q^\top
        \right], 
        \quad
        \numberlabel{2}=\EE\left[
            f(p^h, p^{h'}) L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top W^{h'} x_q x_q^\top 
        \right], \notag\\
        \numberlabel{3}=\EE\left[
            f(p^h, p^{h'}) W^{h} x_q x_q^\top (W^h)^\top L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top W^{h'} x_q x_q^\top
        \right],
        \notag\\
        \numberlabel{4}=\EE\left[
            f(p^h, p^{h'}) W^{h'} x_q x_q^\top (W^h)^\top L_\beta \cT\big(R_\beta (U_Y^h)^\top U_Y^{h'}R_\beta^\top\big) L_\beta^\top W^{h'} x_q x_q^\top
        \right], \notag\\
        \numberlabel{5}=\EE\left[
            f(p^h, p^{h'}) W^{h'} x_q x_q^\top
        \right], 
        \quad 
        \numberlabel{6}=\EE\left[
            f(p^h, p^{h'}) L_\beta \cT\big(R_\beta (U_Y^h)^\top R_\beta^\top\big) L_\beta^\top x_q x_q^\top
        \right], 
        \notag\\
        \numberlabel{7}=\EE\left[
            f(p^h, p^{h'}) W^{h} x_q x_q^\top (W^h)^\top L_\beta \cT\big(R_\beta (U_Y^h)^\top R_\beta^\top\big) L_\beta^\top x_q x_q^\top
        \right], 
    \end{gather*}
    for any $f(p^h, p^{h'})$ that is a function of $p^h$ and $p^{h'}$.
    We use two test vectors $v_{X, i}$ and $v_{X, j}$ to show that all these terms have no cross term for $i\neq j$.
    We first note that both $W^h$ and $L_\beta \cT(\cdot)  L_\beta^\top$ are symmetric and take $v_X$ as their eigen vectors. 
    Thus, for terms $\numberlabel{1}$, $\numberlabel{2}$, $\numberlabel{5}$, and $\numberlabel{6}$, we just need to show that $\EE[f(p^h, p^{h'}) v_{X, i}^\top x_q x_q^\top v_{X, j}] = 0$ for $i\neq j$.
    For the rest, we need to show that $\EE[f(p^h, p^{h'}) v_{X, i}^\top x_q x_q^\top v_{X, j} (v_{X, k}^\top x_q)^2] = 0$ for $i\neq j$ and any $k\in[d_x]$. Here, we only need to consider the squared term of $v_{X, k}$ by noting that the the middle terms $(W^h)^\top L_\beta \cT(\cdot) L_\beta^\top W^{h'}$ and $(W^h)^\top L_\beta \cT(\cdot) L_\beta^\top$ are symmetric and take $v_X$ as their eigen vectors.

    For simplicity, we let $\sigma_q = (v_{X, 1}^\top x_q, \dots, v_{X, d_x}^\top x_q)^\top$, $\sigma_l = (v_{X, 1}^\top x_l, \dots, v_{X, d_x}^\top x_l)^\top$ for any $l\in [L]$, $\lambda_K^h = (\lambda_{K, k}^h)_{k\in[d_x]}$, $\lambda_Q^h = (\lambda_{Q, k}^h)_{k\in[d_x]}$, and define vector $\lambda_W^h= \lambda_{K}^h \odot \lambda_{Q}^h/\sqrt d$.
     We claim that the joint distribution of $p^h, p^{h'}$ is determined merely by $\norm{\lambda_{W}^h \odot \sigma_q}_2^2$, $\norm{\lambda_{W}^{h'} \odot \sigma_q}_2^2$, and $ \langle \lambda_{W}^h \odot \sigma_q, \lambda_{W}^{h'} \odot \sigma_q\rangle$. To see this point, recall that the attention score is given by 
     \begin{align*}
        s_l^h = x_l^\top W^h  x_q = \sigma_l^\top  (\lambda_W^h \odot \sigma_q).
     \end{align*}
     Note that $\{\sigma_l\}_{l\in[L]}$ are i.i.d. Gaussian vectors whose distribution is rotation invariant. Thus, applying any rotation matrix $R\in\RR^{d_x\times d_x}$ to $(\lambda_W^h \odot \sigma_q)$ and $(\lambda_W^{h'} \odot \sigma_q)$ at the same time will not change the joint distribution of $(s^h, s^{h'})$, and hence the joint distribution of $(p^h, p^{h'})$.
     Under the rotation equivalence, we conclude that the joint distribution of $(p^h, p^{h'})$ is determined merely by $\norm{\lambda_{W}^h \odot \sigma_q}_2^2$, $\norm{\lambda_{W}^{h'} \odot \sigma_q}_2^2$, and $ \langle \lambda_{W}^h \odot \sigma_q, \lambda_{W}^{h'} \odot \sigma_q\rangle$. Hence, we can rewrite function $f(p^h, p^{h'})$ as 
     $$f\left(\norm{\lambda_{W}^h \odot \sigma_q}_2^2, \norm{\lambda_{W}^{h'} \odot \sigma_q}_2^2, \langle \lambda_{W}^h \odot \sigma_q, \lambda_{W}^{h'} \odot \sigma_q\rangle\right). $$
     To this end, our task boils down to showing that for any $i\neq j$, 
     \begin{align*}
        &\EE\left[f\left(\norm{\lambda_{W}^h \odot \sigma_q}_2^2, \norm{\lambda_{W}^{h'} \odot \sigma_q}_2^2, \langle \lambda_{W}^h \odot \sigma_q, \lambda_{W}^{h'} \odot \sigma_q\rangle\right)\sigma_{q, i} \sigma_{q, j}\right] = 0, \notag\\
        &\EE\left[f\left(\norm{\lambda_{W}^h \odot \sigma_q}_2^2, \norm{\lambda_{W}^{h'} \odot \sigma_q}_2^2, \langle \lambda_{W}^h \odot \sigma_q, \lambda_{W}^{h'} \odot \sigma_q\rangle\right)\sigma_{q, i} \sigma_{q, j} \sigma_{q, k}^2\right] = 0, \quad \forall k\in[d_x]. \notag
     \end{align*}
     In the above terms, we can apply a transformation to $\sigma_q$ and obtain $\sigma_q'$ such that $\sigma_{q, j}' =  - \sigma_{q, j}$, while the other entries remain the same. 
     We observe that the value of $f$ does not change under this transformation. 
     Moreover, the distribution of $\sigma_q'$ is the same as $\sigma_q$. 
     Hence, 
     \begin{align*}
        &\EE\left[f\left(\norm{\lambda_{W}^h \odot \sigma_q}_2^2, \norm{\lambda_{W}^{h'} \odot \sigma_q}_2^2, \langle \lambda_{W}^h \odot \sigma_q, \lambda_{W}^{h'} \odot \sigma_q\rangle\right)\sigma_{q, i} \sigma_{q, j}\right] \notag\\
        &\quad = \frac 1 2 \biggl(
            \EE\left[f\left(\norm{\lambda_{W}^h \odot \sigma_q}_2^2, \norm{\lambda_{W}^{h'} \odot \sigma_q}_2^2, \langle \lambda_{W}^h \odot \sigma_q, \lambda_{W}^{h'} \odot \sigma_q\rangle\right)\sigma_{q, i} \sigma_{q, j}\right]
            \notag\\
            &\autoquad{3}+ \EE\left[f\left(\norm{\lambda_{W}^h \odot \sigma_q' }_2^2, \norm{\lambda_{W}^{h'} \odot \sigma_q' }_2^2, \langle \lambda_{W}^h \odot \sigma_q' , \lambda_{W}^{h'} \odot \sigma_q' \rangle\right)\sigma_{q, i} \sigma_{q, j}'\right]
        \biggr)  = 0. 
     \end{align*}
    The same argument also applies to the second term. Hence, we have shown that $A_{X, X}^{h}$ is symmetric and can be decomposed onto rank one matrices $\{v_{X, k} (v_{X, k})^\top\}_{k\in[d_x]}$.
     This completes the proof.
\end{proof}

\paragraph{Summary of the Results.}
Previously, we have shown that the dynamics can be reduced to the eigenvalue space. 
We now summarize this reduced dynamics. 
For $O^h$ and $V_{ Y}^h$, we have their eigenvalues $\lambda_O^h\in\RR^{d_y}$, $\lambda_V^h \in \RR^{d_y}$ updated by
\begin{align*}
    \dot \lambda_{O}^h = - \lambda_{B}^h \odot \lambda_{V}^h, \quad \dot \lambda_{V}^h = - \lambda_{B}^h \odot \lambda_{O}^h.
\end{align*}
Here, $\lambda_B^h \in \RR^{d_y}$ is the vector of eigenvalues for $B_Y^h$, which is given by
\begin{align*}
\lambda_{B}^h &=  \sum_{h^{\prime}=1}^{H}\left(\left(\frac{\sigma_{x}^{2}}{d_x d_{y}}  \cdot \mathbb{E}\bigl[(p^{h^{\prime}})^{\top} p^{h}\bigr] \cdot (\tilde G^\top \vone)
+\sigma_{\varepsilon}^{2} \cdot \mathbb{E}\bigl[(p^{h^{\prime}})^{\top} p^{h}\bigr] \vone\right) \odot \lambda_{U}^{h^{\prime}}\right. \\
& \autoquad{2} \color{magenta} + \frac{\sigma_x^4}{d_x d_y} \cdot \mathbb{E}\left[ \Phi_2(p^h, p^{h'})\cdot \tilde G^\top \left(\lambda_{W}^{h'} \odot \lambda_{W}^{h^{\prime}} \odot  \sigma_q^{\odot 2}\right) \right] \odot \lambda_{U}^{h^{\prime}}
\\
& \autoquad{2} \color{magenta} + \frac{\sigma_x^4}{d_x d_y} \cdot \mathbb{E}\left[ \Phi_2(p^h, p^{h'})\cdot \tilde G^\top \left(\lambda_{W}^{h} \odot \lambda_{W}^{h} \odot  \sigma_q^{\odot 2}\right) \right] \odot \lambda_{U}^{h^{\prime}}
\\
& \autoquad{2} \left.+\frac{\sigma_{x}^{4}}{d_x d_y} \cdot
\mathbb{E}\left[ \bigl(1 + \Phi_1(p^h, p^{h'})\bigr)\cdot \tilde G^\top \left(\lambda_{W}^{h} \odot \lambda_{W}^{h^{\prime}} \odot  \sigma_q^{\odot 2}\right) \right] \odot \lambda_{U}^{h^{\prime}}\right) \\
& \autoquad{2} -\frac{\sigma_{x}^{2}}{d_x d_{y}} \cdot \mathbb{E}\left[(1 - \norm{p^h}_2^2)\cdot \tilde G^\top \left(\lambda_{W}^{h} \odot \sigma_{q}^{\odot 2}\right)\right] , 
\end{align*}
where we denote by $\lambda_{U}^h = \lambda_O^h \odot \lambda_V^h $, denote by $\Phi_1(\cdot)$ the term that scales with $L^{-1}$ according to the approximation result in \Cref{lemma: E[pq]-moment}, and by $\Phi_2(\cdot)$ the higher order terms that scales at most $\sqrt{\EE[\Phi_2^2]} \le L^{-1.25}$ according to \Cref{lemma: higher-order-moment}.
Note that in the above equation, under the condition that $\lambda_W^h \le \cO(d^{-1/2})$, we can we can always merge the higher order term containing $\Phi_2(\cdot)$ with some lower order terms, at the cost of introducing a higher order error. For instance, we can merge the term $\EE[\Phi_2(p^h, p^{h'})\cdot \tilde G^\top (\lambda_{W}^{h'} \odot \lambda_{W}^{h^{\prime}} \odot  \sigma_q^{\odot 2})]$ with the first term and add a multiplier $(1+\cO(L^{-1.25}))$ to each coordinate of $\lambda_B^h$. For this very reason, we refrain ourselves from the complication by ignoring the higher order term $\Phi_2(\cdot)$ in the following analysis.

Similarly for $K_{ X}^h$ and $Q_{ X}^h$, we have their eigenvalues $\lambda_K^h\in\RR^{d_x}$ and $\lambda_Q^h\in\RR^{d_x}$ updated by
\begin{align*}
    \dot \lambda_{K}^h = - \frac{1}{\sqrt d} \lambda_{A}^h \odot \lambda_{Q}^h, \quad \dot \lambda_{Q}^h = - \frac{1}{\sqrt d}\lambda_{A}^h \odot \lambda_{K}^h, 
\end{align*}
where $\lambda_A^h\in\RR^{d_x}$ is the vector of eigenvalues of $A_{X, X}^h$.
Let $\lambda_W^h = \lambda_K^h \odot \lambda_Q^h/\sqrt d$. 
Then, $\lambda_A^h$ admits the following decomposition $\lambda_A^h = \sum_{h'=1}^H (\lambda_{A, \signal}^{h, h'} + \lambda_{A, \noise}^{h, h'}) + \lambda_A^{h, 0}$ with $\lambda_{A, \signal}^{h, h'}$ given by
$$
\begin{aligned}
\lambda_{A, \signal}^{h, h^{\prime}}
& \approx \frac{1}{d_{x} d_{y}} \cdot\biggl(
    \sigma_{x}^{4} \left(\vone^\top \tilde G (\lambda_{U}^h \odot \lambda_{U}^{h'})\right) \cdot \mathbb{E}\left[
        (p^{h})^{\top} p^{h^{\prime}} \sigma_q^{\odot 2}\right] \odot \lambda_{W}^{h^{\prime}} 
        \\
& \autoquad{3} + \sigma_{x}^{4} \EE\left[\bigl(1 - \norm{p^h}_2^2 - \norm{p^{h}}_2^2 + (p^h)^\top p^{h'}\bigr) \cdot \sigma_q^{\odot 2}\right] 
        \odot \left(\tilde G (\lambda_{U}^{h} \odot \lambda_{U}^{h'})\right) \odot \lambda_{W}^{h^{\prime}}
    \\
& \autoquad{3} +\sigma_{x}^{6} \mathbb{E}\left[-2\|p^{h}\|_{2}^{2}
    \cdot \left\langle\lambda_{W}^{h} 
    \odot \lambda_{W}^{h^{\prime}} \left(\tilde G (\lambda_{U}^h\odot \lambda_{U}^{h'}) \right), \sigma_{q}^{\odot 2}\right\rangle 
    \cdot \sigma_{q}^{\odot 2}\right] \odot \lambda_{W}^{h} \\
& \autoquad{3} +\sigma_{x}^{6} \mathbb{E}\left[
        (p^{h})^{\top} p^{h^{\prime}} 
        \cdot \left\langle\lambda_{W}^{h} 
        \odot \lambda_{W}^{h^{\prime}} \left(\tilde G (\lambda_{U}^h\odot \lambda_{U}^{h'}) \right), \sigma_{q}^{\odot 2}\right\rangle 
        \cdot \sigma_{q}^{\odot {2}}\right] \odot \lambda_{W}^{h^{\prime}}
    \biggr),
\end{aligned}
$$
and $\lambda_{A, \noise}^{h, h'}$ given by
\begin{align*}
\lambda_{A, \noise}^{h, h^{\prime}} \approx \sigma_{\varepsilon}^{2} \sigma_{x}^{2} \cdot \mathbb{E}\left[
    (p^{h})^{\top} p^{h^{\prime}} 
    \cdot \bigl\langle\lambda_{U}^{h}, \lambda_{U}^{h^{\prime}}\bigr\rangle 
    \cdot \sigma_{q}^{\odot {2}} \odot \lambda_{W}^{h^{\prime}}
    \right], 
\end{align*}
and $\lambda_A^{h, 0}$ given by
$$
\begin{aligned}
& \lambda_{A}^{h, 0}=\frac{1}{d_x d_y}         
    \cdot 
        \mathbb{E}\left[
            -\sigma_{x}^{2}  \bigl(1-\|p^{h}\|_{2}^{2}\bigr)\cdot \sigma_{q}^{\odot 2} \odot (\tilde G \lambda_{U}^h)
            + 2 \sigma_{x}^{4}(\|p^{h}\|_{2}^{2} + \Phi_2(p^h)) \cdot \bigl\langle (\tilde G \lambda_{U}^h) \odot \lambda_{W}^{h}, \sigma_{q}^{\odot 2}\bigr\rangle \cdot \sigma_{q}^{\odot 2} \odot \lambda_{W}^{h}\right] 
     .
\end{aligned}
$$
Here, the \say{$\approx$} in both $\lambda_{A, \signal}^{h, h'}$ and $\lambda_{A, \noise}^{h, h'}$ hides (i) higher order term with respect to $p^h$ and $p^{h'}$ and (ii) higher order term with respect to $\lambda_W^h$ or $(\lambda_1, \lambda_2, \lambda_3) \in \{\lambda_W^h, \lambda_W^{h'}\}^3 \backslash \{(\lambda_W^h, \lambda_W^{h'}, \lambda_W^h)\cup (\lambda_W^h, \lambda_W^{h'},\lambda_W^{h'})\}$. 


==> sections/paperlogic.tex <==
{\color{violet}\vspace{1cm}
\noindent\textbf{
TODO: 
\begin{myenumi}
\item change corpus to task
\item Discussion of the peak in the dynamics curves for $L/d<1$ and $L/d>1$
\item Yuanzhi's knowledge distillation \url{https://arxiv.org/pdf/2012.09816.pdf}
\end{myenumi}
}
}

\section{Paper Logic}
\begin{myenumi}
    \item (Preliminaries) We consider a multi-head softmax attention mechanism trained on multi-task linear regression data where we run gradient descent under the L2 population loss. 
    \item (Global optimality for single-head multiple task) We should first understand the global optimality of a single-head attention trained for multi-task since: 
    \begin{myenumi}
        \item It is the simplest case and gives us a sense of how the attention mechanism conducts icl.
        \item It provides the optimal scaling for the attention weights ($\ll \sqrt{2\log L}$), building upon which we can further our analysis. 
    \end{myenumi}
    \item (Decomposable Weights) Analyzing the training dynamics from arbitrary initialization is too challenging due to the non-convexity in the softmax attention mechanism and the coupling between the attention weights. 
    \begin{myenumi}
        \item To simplify the problem while distilling the essential elements, we consider a class of decomposable weights, and show that if initialized within the class, the decomposable property is preserved. 
        \item To justify the use of decomposable weights, we argue by: (1) it is a natural choice (perhaps optimal) to project the key and query into the covariate $X$'s subspace, while letting the value to be within the $Y$'s subspace (we cannot give a rigorous proof for this argument, but this is a common practice in the literature, e.g., \citep{zhang2023trained}) (2) Based on the proof for optimality in the single task's case, we further prove that for a single head and multi-task, the optimal $U_Y, W_X$ are decomposable. 
        \item With decomposability, we can consider all the weights to be diagonal, with $q, k, v, o$ to be the vectors of the diagonal elements of $Q, K, V, O$ respectively.
    \end{myenumi}
    \item (Training Dynamics for Single Head Single Task) We analyze the training dynamics for single head single task with $q=k, v=o$ (WLOG by global optimality) and show (1) convergence to the global optimum (2) the emergence of the skill.  \Siyu{Perhaps we can extend to single head multi-task? haven't done the math yet.}
    \item (Training Dynamics for Multi-head Multi-tasks) We consider $H$ heads and $I$ tasks. Since $q=k, v=o$ results in $\mu, \omega$ to be non-negative, and the optimal solution for multi-head case is not necessarily all positive eigenvalues, we need to consider the following two cases:
    \begin{myenumi}
        \item (Symmetric Weights) With $q=k, v=o$ at initialization, suppose $H \ge I$, we have convergence to the solution where each task is completed by an individual head in the manner described in the case of single head single task.
        \item (Asymmetric Weights) With $q\neq k, v\neq o$ at initialization, suppose $H = I$, we find empirically that the attention weights converge to a different solution {\color{red} [give a $H=3$ experiment result?]}. Theoretically, we find a class of solutions that gives the same icl loss where (1) $\{\baromega^\h\}_{h\in[H]}$ lies on a $H$-dimensional sphere centered at the origin with the same angle between each pair of $\baromega^\h$'s (Maybe we can call it equiangular line systems?) (2) $\sum_{h\in[H]} \baromega^\h=0$. We prove that
        \begin{myenumi}
            \item Any rotation of the solution has the same icl loss. 
            \item Within the class of equiangular line systems of size $H$ dimension $H$, solutions satisfying (2) $\sum_{h\in[H]} \baromega^\h=0$ are the global optimum.
            \item \todo{Can we show convergence with asymmetric weights? Starting from zero initialization but satisfying the equiangular line constraint? Already verified by experiments, think it should not be too hard. }
    \end{myenumi}
    \item (Comparison between symmetric and asymmetric weights) Consider $H=I$. 
    \begin{myenumi} 
        \item The \say{equiangular line systems} solution gives a better icl rate than the symmetric weights solution. 
        \item The symmetric weights solution can be viewed as a collection of \say{subsystems} where each task is handled independently by a head. Though not optimal, it still implements the enrolled optimization structure demonstrated in \citep{yu2023white}.
        \item The asymmetric weights solution highlights a \say{coorperation} among heads, where each task is first distributed among the heads and then by properly aggregating the outputs from all the heads, the tasks are completed.
    \end{myenumi}
    \end{myenumi}
\end{myenumi}


\begin{center}
    \begin{tabular}{l@{\hspace{1cm}}p{6cm}}
        \hline
        \hline
        \textbf{Notations} & \textbf{Objects} \\
        \hline
        $H, L$ & Number of heads, sequence length\\
        $d, d_y, D=d+d_y, d_e$ & Dim of covariate, label, and $d_e$ is the embedding dimension\\
        $Q^\h, K^\h, V^\h, O^\h$ & Query, key, value, output \\
        $W^\h={K^\h}^\top Q^\h$, $U^\h = O^\h V^\h$ &  \\
        $\omega^\h, \mu^\h; \omega^\h_{i}, \mu^\h_{i}$ & Singular values of $W$ and $U$ and for each task $i$ and each head $h$ \\
        $Z, X, Y, z_q; x_l, y_l, q, y_q; \hat y$ & data (for position $l$, where we can safely use the subscript for position)\\
        $i \in [I], d_i$ & Tasks and task-wise dimension\\
        $\lambda \in \RR^I, \sigma^2$ & Strength of signals, variance of noise\\
        $\mathrm{SNR}_i = \frac{}{}, \phi = (1+\mathrm{SNR}_1^{-1}, \ldots, 1 + \mathrm{SNR}_I^{-1})^\top$ & \\
        $s^\h = \frac{Z^\top {K^\h}^\top Q^\h z_q}{\sqrt{d_e}}$ & \\
        $p^\h = \mathrm{softmax}(s^\h)$ & \\
        $P^\h = \diag(p^\h) - p^\h {p^\h}^\top$ & \\
        $G = \frac{1}{\sqrt{d_e}} \varPhi \overbar G \varPsi^\top$, $\EE[\overbar G\overbar G^\top]=\varLambda$ & Use $G$ to avoid conflict with $A, B$ used for dynamics.\\ 
        $\check q = \varPhi^\top q $ & \\
        \hline
        \hline
    \end{tabular}
\end{center}
